Advancing Fine-Grained Classification by Structure and Subject Preserving Augmentation

Fine-grained visual classification (FGVC) involves classifying closely related sub-classes. This task is difficult due to the subtle differences between classes and the high intra-class variance. Moreover, FGVC datasets are typically small and challenging to gather, thus highlighting a significant need for effective data augmentation. Recent advancements in text-to-image diffusion models offer new possibilities for augmenting classification datasets. While these models have been used to generate training data for classification tasks, their effectiveness in full-dataset training of FGVC models remains under-explored. Recent techniques that rely on Text2Image generation or Img2Img methods, often struggle to generate images that accurately represent the class while modifying them to a degree that significantly increases the dataset's diversity. To address these challenges, we present SaSPA: Structure and Subject Preserving Augmentation. Contrary to recent methods, our method does not use real images as guidance, thereby increasing generation flexibility and promoting greater diversity. To ensure accurate class representation, we employ conditioning mechanisms, specifically by conditioning on image edges and subject representation. We conduct extensive experiments and benchmark SaSPA against both traditional and recent generative data augmentation methods. SaSPA consistently outperforms all established baselines across multiple settings, including full dataset training, contextual bias, and few-shot classification. Additionally, our results reveal interesting patterns in using synthetic data for FGVC models; for instance, we find a relationship between the amount of real data used and the optimal proportion of synthetic data. Code is available at https://github.com/EyalMichaeli/SaSPA-Aug.

==> ablations.tex <==

\subsection{Effect of Different Generation Strategies on Performance}
\label{sec:mai_ablation}
In \Cref{tab:main_ablation}, we conduct an extensive ablation study to evaluate the effectiveness of our proposed generation strategies. Specifically, we examine the integration of edge guidance, Img2Img as an alternative for edge guidance with strength = $0.5$ and in combination with edge guidance with strength = $0.85$, and subject representation. We also investigate the effect of using the same image for both edges extraction and the subject reference image (``Edges=Ref.''). 
Additionally, we test the impact of appending half of the prompts with artistic styles (column `Art.') as described in \Cref{subsec:diff_prompts}.
\input{tbls/ablations/main_ablation}

\textbf{The results} 
demonstrate the importance of combining structural and subject-level conditioning while enabling diverse generations through separate input sources, yielding the best performance across most datasets.
Key observations include: (1) Edge Guidance alone improves performance significantly compared to Text-to-Image or SDEdit \cite{meng2021sdedit} (Img2Img), highlighting its important role in providing structural guidance. (2) Subject representation alone does not enhance performance, indicating additional structural conditioning is necessary. (3) Using different source images for edges and subject reference images adds beneficial diversity. (4) Surprisingly, text-to-image generation (first row) outperforms SDEdit, likely due to its increased diversity and despite the lower fidelity, which our filtering mechanism can handle as it filters out low-fidelity images. (5) Incorporating artistic prompts has inconsistent effects, usually boosting performance with Edge Guidance but often degrading it when combined with subject representation. This inconsistency may stem from the fact that subject representation uses BLIP-diffusion \cite{li2024blipdiffusion}, which is a different base model than Stable Diffusion \cite{rombach2022high}, as Stable Diffusion is fine-tuned. Additionally, in CUB, artistic prompts offer no improvement even when using Edge Guidance without subject representation, likely due to the dataset's heavy reliance on color as a primary discriminator between bird types, potentially disrupted by artistic prompts.


